Classifying Galaxy Morphologies with Few-Shot Learning

The taxonomy of galaxy morphology is critical in astrophysics as the morphological properties are powerful tracers of galaxy evolution. With the upcoming Large-scale Imaging Surveys, billions of galaxy images challenge astronomers to accomplish the classification task by applying traditional methods or human inspection. Consequently, machine learning, in particular supervised deep learning, has been widely employed to classify galaxy morphologies recently due to its exceptional automation, efficiency, and accuracy. However, supervised deep learning requires extensive training sets, which causes considerable workloads; also, the results are strongly dependent on the characteristics of training sets, which leads to biased outcomes potentially. In this study, we attempt Few-shot Learning to bypass the two issues. Our research adopts the dataset from Galaxy Zoo Challenge Project on Kaggle, and we divide it into five categories according to the corresponding truth table. By classifying the above dataset utilizing few-shot learning based on Siamese Networks and supervised deep learning based on AlexNet, VGG_16, and ResNet_50 trained with different volumes of training sets separately, we find that few-shot learning achieves the highest accuracy in most cases, and the most significant improvement is $21\%$ compared to AlexNet when the training sets contain 1000 images. In addition, to guarantee the accuracy is no less than 90\%, few-shot learning needs $\sim$6300 images for training, while ResNet_50 requires 13000 images. Considering the advantages stated above, foreseeably, few-shot learning is suitable for the taxonomy of galaxy morphology and even for identifying rare astrophysical objects, despite limited training sets consisting of observational data only.

==> readme <==
Dear Colleagues: 

The final publication layout will be produced by using raa.cls. 
Therefore, we strongly encourage you to prepare your LaTeX manuscript 
with this class file. Please unpack raa-package.tar.gz, it includes 

raa.cls        ---- RAA macro class file for LaTeX2e 
sample.tex     ---- a sample file using raa.cls (LaTeX source) 
sample.ps      ---- the PS file created by sample.tex in referee format  
sample.pdf     ---- the PDF file created by sample.tex in referee format  
readme         ---- this file  
f?.eps         ---- three demo figures used in the LaTeX template source
sample2.tex    ---- a sample file for using raa.bst
sample2_fig?.eps -- two demo figures used in sample2.tex
sample2.pdf    ---- the PDF file created by sample.tex in referee format
sample2.bbl    ---- bibliography file using by sample2.tex
bibtex.bib     ---- an example for bibtex file

natbib.sty     ---- This package reimplements the LaTeX \cite command
natnotes.pdf   ---- Brief reference sheet for Natbib (pdf)
raa.bst        ---- Bibliography style file 

Hope you enjoy the use of this macro. Your suggestions and comments are 
highly welcome. Thanks.

Editorial Office
E-mail:  raa@raa-journal.org

